Degeneration of Topological String partition functions and Mirror curves of the Calabi-Yau threefolds $X_{N,M}$

In this paper we study certain degenerations of the mirror curves, associated with Calabi-Yau threefolds $X_{N,M}$, and the effect of these degenerations on the topological string partition function of $X_{N,M}$. We show that when the mirror curve degenerates and become the union of the lower genus curves the corresponding partition function factorizes into pieces corresponding to the components of the degenerate mirror curve. Moreoever we show that using degeneration of a generalised mirror curve it is possible to obtain the partition function corresponding to $X_{N,M-1}$ from $X_{N,M}$.

==> bibliography.tex <==
@article{Koroteev:2019gqi,
    author = "Koroteev, Peter and Shakirov, Shamil",
    title = "{The Quantum DELL System}",
    eprint = "1906.10354",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s11005-019-01247-y",
    journal = "Lett. Math. Phys.",
    volume = "110",
    pages = "969--999",
    year = "2020"
}

@article{Alvarez-Gaume_166751,
      author        = "Alvarez-Gaume, Luis and Moore, G and Vafa, C",
      title         = "{Theta functions, modular invariance, and strings}",
      journal       = "Commun. Math. Phys.",
      reportNumber  = "HUTP-86-A-017",
      volume        = "106",
      pages         = "1. 73 p",
      month         = "Mar",
      year          = "1986",
      url           = "https://cds.cern.ch/record/166751",
}
@article{Strominger:1996it,
    author = "Strominger, Andrew and Yau, Shing-Tung and Zaslow, Eric",
    title = "{Mirror symmetry is T duality}",
    eprint = "hep-th/9606040",
    archivePrefix = "arXiv",
    doi = "10.1016/0550-3213(96)00434-8",
    journal = "Nucl. Phys. B",
    volume = "479",
    pages = "243--259",
    year = "1996"
}
@article{Aganagic:2001nx,
    author = "Aganagic, Mina and Klemm, Albrecht and Vafa, Cumrun",
    title = "{Disk instantons, mirror symmetry and the duality web}",
    eprint = "hep-th/0105045",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-01-A023, HU-EP-01-21",
    doi = "10.1515/zna-2002-1-201",
    journal = "Z. Naturforsch. A",
    volume = "57",
    pages = "1--28",
    year = "2002"
}
@article{Iqbal:2001kk,
    author = "Iqbal, Amer and Kashani-Poor, Amir-Kian",
    title = "{Discrete symmetries of the superpotential and calculation of disk invariants}",
    eprint = "hep-th/0109214",
    archivePrefix = "arXiv",
    reportNumber = "UTTG-15-01",
    doi = "10.4310/ATMP.2001.v5.n4.a1",
    journal = "Adv. Theor. Math. Phys.",
    volume = "5",
    pages = "651--678",
    year = "2002"
}
@article{Bouchard:2007ys,
    author = "Bouchard, Vincent and Klemm, Albrecht and Marino, Marcos and Pasquetti, Sara",
    title = "{Remodeling the B-model}",
    eprint = "0709.1453",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "BONN-TH-2007-07, CERN-PH-TH-2007-153, NEIP-07-03",
    doi = "10.1007/s00220-008-0620-4",
    journal = "Commun. Math. Phys.",
    volume = "287",
    pages = "117--178",
    year = "2009"
}
@article{Aganagic:2000gs,
    author = "Aganagic, Mina and Vafa, Cumrun",
    title = "{Mirror symmetry, D-branes and counting holomorphic discs}",
    eprint = "hep-th/0012041",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-00-A047",
    month = "12",
    year = "2000"
}
@article{Jefferson_2018,
   title={On geometric classification of 5d SCFTs},
   volume={2018},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP04(2018)103},
   DOI={10.1007/jhep04(2018)103},
   number={4},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Jefferson, Patrick and Katz, Sheldon and Kim, Hee-Cheol and Vafa, Cumrun},
   year={2018},
   month={Apr}
}
@article{Chen:2020jla,
    author = "Chen, Jin and Haghighat, Babak and Kim, Hee-Cheol and Sperling, Marcus",
    title = "{Elliptic Quantum Curves of Class $\mathcal{S}_k$}",
    eprint = "2008.05155",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2020"
}
@article{Jafarzade:2017fsc,
    author = "Jafarzade, Shahriyar and Nazari, Zainab",
    title = "{A New Integrable Ising-type Model from 2d $\mathcal{N}$=(2,2) Dualities}",
    eprint = "1709.00070",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2017"
}
@article{Deger:2018kur,
    author = "Deger, N.S. and Nazari, Z. and Sarioglu, O.",
    title = "{Supersymmetric solutions of N=(1,1) general massive supergravity}",
    eprint = "1803.06926",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.97.106022",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "10",
    pages = "106022",
    year = "2018"
}
@article{Marshakov_2000,
   title={Duality in integrable systems and generating functions for new hamiltonians},
   volume={476},
   ISSN={0370-2693},
   url={http://dx.doi.org/10.1016/S0370-2693(00)00076-9},
   DOI={10.1016/s0370-2693(00)00076-9},
   number={3-4},
   journal={Physics Letters B},
   publisher={Elsevier BV},
   author={Marshakov, A.},
   year={2000},
   month={Mar},
   pages={420?426}
}
@article{Bershadsky_1994,
   title={Kodaira-Spencer theory of gravity and exact results for quantum string amplitudes},
   volume={165},
   ISSN={1432-0916},
   url={http://dx.doi.org/10.1007/BF02099774},
   DOI={10.1007/bf02099774},
   number={2},
   journal={Communications in Mathematical Physics},
   publisher={Springer Science and Business Media LLC},
   author={Bershadsky, M. and Cecotti, S. and Ooguri, H. and Vafa, C.},
   year={1994},
   month={Oct},
   pages={311?427}
}

@article{Friedan:1986ua,
    author = "Friedan, Daniel and Shenker, Stephen H.",
    title = "{The Analytic Geometry of Two-Dimensional Conformal Field Theory}",
    reportNumber = "EFI-86-18A-CHICAGO",
    doi = "10.1016/0550-3213(87)90418-4",
    journal = "Nucl. Phys. B",
    volume = "281",
    pages = "509--545",
    year = "1987"
}
@article{Friedan:1986hr,
    author = "Friedan, D.",
    editor = "Brink, L. and Marnelius, R. and Nilsson, J.S. and Salomonson, P. and Skagerstam, B.S.",
    title = "{A NEW FORMULATION OF STRING THEORY}",
    reportNumber = "EFI-86-52-CHICAGO",
    doi = "10.1088/0031-8949/1987/T15/009",
    journal = "Phys. Scripta T",
    volume = "15",
    pages = "78",
    year = "1987"
}

@article{Hohenegger_2017,
   title={Dual little strings from F-theory and flop transitions},
   volume={2017},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP07(2017)112},
   DOI={10.1007/jhep07(2017)112},
   number={7},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong},
   year={2017},
   month={Jul}
}


@article{Haghighat_2014,
   title={Orbifolds of M-strings},
   volume={89},
   ISSN={1550-2368},
   url={http://dx.doi.org/10.1103/PhysRevD.89.046003},
   DOI={10.1103/physrevd.89.046003},
   number={4},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Haghighat, Babak and Kozcaz, Can and Lockhart, Guglielmo and Vafa, Cumrun},
   year={2014},
   month={Feb}
}

@article{Haghighat_2014,
   title={M-Strings},
   volume={334},
   ISSN={1432-0916},
   url={http://dx.doi.org/10.1007/s00220-014-2139-1},
   DOI={10.1007/s00220-014-2139-1},
   number={2},
   journal={Communications in Mathematical Physics},
   publisher={Springer Science and Business Media LLC},
   author={Haghighat, Babak and Iqbal, Amer and Kozcaz, Can and Lockhart, Guglielmo and Vafa, Cumrun},
   year={2014},
   month={Aug},
   pages={779?842}
}
@article{Bhardwaj_2016,
   title={F-theory and the classification of little strings},
   volume={93},
   ISSN={2470-0029},
   url={http://dx.doi.org/10.1103/PhysRevD.93.086002},
   DOI={10.1103/physrevd.93.086002},
   number={8},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Bhardwaj, Lakshya and Del Zotto, Michele and Heckman, Jonathan J. and Morrison, David R. and Rudelius, Tom and Vafa, Cumrun},
   year={2016},
   month={Apr}
}
@article{Hohenegger:2016eqy,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Self-Duality and Self-Similarity of Little String Orbifolds}",
    eprint = "1605.02591",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.94.046006",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "4",
    pages = "046006",
    year = "2016"
}

@article{Hohenegger_2016,
   title={Instanton-monopole correspondence from M-branes onS1and little string theory},
   volume={93},
   ISSN={2470-0029},
   url={http://dx.doi.org/10.1103/PhysRevD.93.066016},
   DOI={10.1103/physrevd.93.066016},
   number={6},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong},
   year={2016},
   month={Mar}
}
@misc{katz1997mirror,
    title={Mirror symmetry and Exact Solution of 4D N=2 Gauge Theories I},
    author={S. Katz and P. Mayr and C. Vafa},
    year={1997},
    eprint={hep-th/9706110},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}
@article{KONISHI_2008,
   title={FLOP INVARIANCE OF THE TOPOLOGICAL VERTEX},
   volume={19},
   ISSN={1793-6519},
   url={http://dx.doi.org/10.1142/S0129167X08004546},
   DOI={10.1142/s0129167x08004546},
   number={01},
   journal={International Journal of Mathematics},
   publisher={World Scientific Pub Co Pte Lt},
   author={KONISHI, YUKIKO and MINABE, SATOSHI},
   year={2008},
   month={Jan},
   pages={27?45}
}
@misc{bousseau2020holomorphic,
    title={Holomorphic anomaly equation for $(\mathbb{P}^2,E)$ and the Nekrasov-Shatashvili limit of local $\mathbb{P}^2$},
    author={Pierrick Bousseau and Honglu Fan and Shuai Guo and Longting Wu},
    year={2020},
    eprint={2001.05347},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}

@misc{liu2005transformation,
    title={Transformation of algebraic Gromov-Witten invariants of three-folds under flops and small extremal transitions, with an appendix from the stringy and the symplectic viewpoint},
    author={Chien-Hao Liu and Shing-Tung Yau},
    year={2005},
    eprint={math/0505084},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}

@misc{li1998symplectic,
    title={Symplectic surgery and Gromov-Witten invariants of Calabi-Yau 3-folds I},
    author={An-Min Li and Yongbin Ruan},
    year={1998},
    eprint={math/9803036},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}

@misc{taki2008flop,
    title={Flop Invariance of Refined Topological Vertex and Link Homologies},
    author={Masato Taki},
    year={2008},
    eprint={0805.0336},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}

@article{Aharony_1998,
   title={Webs of (p,q) 5-branes, five dimensional field theories and grid diagrams},
   volume={1998},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1088/1126-6708/1998/01/002},
   DOI={10.1088/1126-6708/1998/01/002},
   number={01},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Aharony, Ofer and Hanany, Amihay and Kol, Barak},
   year={1998},
   month={Jan},
   pages={002}
}
@article{Cecotti_2014,
   title={tt * geometry in 3 and 4 dimensions},
   volume={2014},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP05(2014)055},
   DOI={10.1007/jhep05(2014)055},
   number={5},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Cecotti, Sergio and Gaiotto, Davide and Vafa, Cumrun},
   year={2014},
   month={May}
}

@misc{leung1997branes,
    title={Branes and Toric Geometry},
    author={N. C. Leung and C. Vafa},
    year={1997},
    eprint={hep-th/9711013},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}
@misc{kanazawa2016local,
    title={Local Calabi-Yau manifolds of type \tilde{A} via SYZ mirror symmetry},
    author={Atsushi Kanazawa and Siu-Cheong Lau},
    year={2016},
    eprint={1605.00342},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}

@article{Bershadsky_1996,
   title={Geometric singularities and enhanced gauge symmetries},
   volume={481},
   ISSN={0550-3213},
   url={http://dx.doi.org/10.1016/S0550-3213(96)90131-5},
   DOI={10.1016/s0550-3213(96)90131-5},
   number={1-2},
   journal={Nuclear Physics B},
   publisher={Elsevier BV},
   author={Bershadsky, M. and Intriligator, K. and Kachru, S. and Morrison, D.R. and Sadov, V. and Vafa, C.},
   year={1996},
   month={Dec},
   pages={215-252}
}

@article{Aganagic_2004,
   title={The Topological Vertex},
   volume={254},
   ISSN={1432-0916},
   url={http://dx.doi.org/10.1007/s00220-004-1162-z},
   DOI={10.1007/s00220-004-1162-z},
   number={2},
   journal={Communications in Mathematical Physics},
   publisher={Springer Science and Business Media LLC},
   author={Aganagic, Mina and Klemm, Albrecht and Marino, Marcos and Vafa, Cumrun},
   year={2004},
   month={Sep},
   pages={425-478}
}
@article{Iqbal_2009,
   title={The refined topological vertex},
   volume={2009},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1088/1126-6708/2009/10/069},
   DOI={10.1088/1126-6708/2009/10/069},
   number={10},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Iqbal, Amer and Kozcaz, Can and Vafa, Cumrun},
   year={2009},
   month={Oct},
   pages={069-069}
}

@article{Hohenegger_2014,
   title={M-strings, elliptic genera andN= 4 string amplitudes},
   volume={62},
   ISSN={0015-8208},
   url={http://dx.doi.org/10.1002/prop.201300035},
   DOI={10.1002/prop.201300035},
   number={3},
   journal={Fortschritte der Physik},
   publisher={Wiley},
   author={Hohenegger, S. and Iqbal, A.},
   year={2014},
   month={Feb},
   pages={155?206}
}
@article{Hohenegger_2015,
   title={M-strings, monopole strings, and modular forms},
   volume={92},
   ISSN={1550-2368},
   url={http://dx.doi.org/10.1103/PhysRevD.92.066005},
   DOI={10.1103/physrevd.92.066005},
   number={6},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong},
   year={2015},
   month={Sep}
}
@article{Braden:2003gv,
    author = "Braden, Harry W. and Hollowood, Timothy J.",
    title = "{The Curve of compactified 6-D gauge theories and integrable systems}",
    eprint = "hep-th/0311024",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2003/12/023",
    journal = "JHEP",
    volume = "12",
    pages = "023",
    year = "2003"
}

@article{Hollowood_2008,
   title={Matrix models, geometric engineering and elliptic genera},
   volume={2008},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1088/1126-6708/2008/03/069},
   DOI={10.1088/1126-6708/2008/03/069},
   number={03},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Hollowood, Timothy and Iqbal, Amer and Vafa, Cumrun},
   year={2008},
   month={Mar},
   pages={069?069}
}
@misc{nekrasov2002seibergwitten,
    title={Seiberg-Witten Prepotential From Instanton Counting},
    author={Nikita A. Nekrasov},
    year={2002},
    eprint={hep-th/0206161},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}

@article{Witten:1986bf,
    author = "Witten, Edward",
    title = "{Elliptic Genera and Quantum Field Theory}",
    reportNumber = "PUPT-1024",
    doi = "10.1007/BF01208956",
    journal = "Commun. Math. Phys.",
    volume = "109",
    pages = "525",
    year = "1987"
}
@article{Lerche:1987qk,
    author = "Lerche, W. and Nilsson, B.E.W. and Schellekens, A.N. and Warner, N.P.",
    title = "{Anomaly Cancelling Terms From the Elliptic Genus}",
    reportNumber = "CERN-TH-4765/87",
    doi = "10.1016/0550-3213(88)90468-3",
    journal = "Nucl. Phys. B",
    volume = "299",
    pages = "91--116",
    year = "1988"
}
@article{NAB:2020N,
    author = "Ambreen Ahmed,M.Nouman Muteeb",
    title = "{in preparation}",
}

@article{Aharony_2000,
   title={A brief review of `little string theories'},
   volume={17},
   ISSN={1361-6382},
   url={http://dx.doi.org/10.1088/0264-9381/17/5/302},
   DOI={10.1088/0264-9381/17/5/302},
   number={5},
   journal={Classical and Quantum Gravity},
   publisher={IOP Publishing},
   author={Aharony, Ofer},
   year={2000},
   month={Feb},
   pages={929--938}
}
@misc{huang2010direct,
    title={Direct integration for general Omega backgrounds},
    author={Min-xin Huang and Albrecht Klemm},
    year={2010},
    eprint={1009.1126},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}
@article{Huang:2011qx,
    author = "Huang, Min-xin and Kashani-Poor, Amir-Kian and Klemm, Albrecht",
    title = "{The $\Omega$ deformed B-model for rigid $\mathcal{N}=2$ theories}",
    eprint = "1109.5728",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IPMU10-0162, BONN-TH-2011-13, LPTENS-11-38",
    doi = "10.1007/s00023-012-0192-x",
    journal = "Annales Henri Poincare",
    volume = "14",
    pages = "425--497",
    year = "2013"
}

@article{Hellerman_2012,
   title={String theory of the Omega deformation},
   volume={2012},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP01(2012)148},
   DOI={10.1007/jhep01(2012)148},
   number={1},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Hellerman, Simeon and Orlando, Domenico and Reffert, Susanne},
   year={2012},
   month={Jan}
}
@article{Gopakumar:1998ii,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 1.}",
    eprint = "hep-th/9809187",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A069",
    month = "9",
    year = "1998"
}
@article{Gopakumar:1998jq,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 2.}",
    eprint = "hep-th/9812127",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A070",
    month = "12",
    year = "1998"
}
@misc{gopakumar1998mtheory,
    title={M-Theory and Topological Strings--I},
    author={Rajesh Gopakumar and Cumrun Vafa},
    year={1998},
    eprint={hep-th/9809187},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}

@misc{gopakumar1998mtheory,
    title={M-Theory and Topological Strings--II},
    author={Rajesh Gopakumar and Cumrun Vafa},
    year={1998},
    eprint={hep-th/9812127},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}
@book{Eichler2013TheTO,
 title={The Theory of Jacobi Forms},
  author={M. Eichler and D. Zagier}
}

@misc{lockhart2012superconformal,
    title={Superconformal Partition Functions and Non-perturbative Topological Strings},
    author={Guglielmo Lockhart and Cumrun Vafa},
    year={2012},
    eprint={1210.5909},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}

@misc{kawai2000string,
    title={String Partition Functions and Infinite Products},
    author={Toshiya Kawai and Kota Yoshioka},
    year={2000},
    eprint={hep-th/0002169},
    archivePrefix={arXiv},
    primaryClass={hep-th}
}

@article{Ahmed_2017,
   title={Bound states of little strings and symmetric orbifold conformal field theories},
   volume={96},
   ISSN={2470-0029},
   url={http://dx.doi.org/10.1103/PhysRevD.96.081901},
   DOI={10.1103/physrevd.96.081901},
   number={8},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Ahmed, Ambreen and Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong},
   year={2017},
   month={Oct}
}

@article{Haghighat_2019,
   title={M5 branes and theta functions},
   volume={2019},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP10(2019)192},
   DOI={10.1007/jhep10(2019)192},
   number={10},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Haghighat, Babak and Sun, Rui},
   year={2019},
   month={Oct}
}

@article{Harvey_2015,
   title={Elliptic genera of ALE and ALF manifolds from gauged linear sigma models},
   volume={2015},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP02(2015)110},
   DOI={10.1007/jhep02(2015)110},
   number={2},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Harvey, Jeffrey A. and Lee, Sungjay and Murthy, Sameer},
   year={2015},
   month={Feb}
}
@misc{bryan2019donaldsonthomas,
    title={The Donaldson-Thomas partition function of the banana manifold},
    author={Jim Bryan},
    year={2019},
    eprint={1902.08695},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}

@article{Dijkgraaf_2008,
   title={Supersymmetric gauge theories, intersecting branes and free fermions},
   volume={2008},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1088/1126-6708/2008/02/106},
   DOI={10.1088/1126-6708/2008/02/106},
   number={02},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Dijkgraaf, Robbert and Hollands, Lotte and Sulkowski, Piotr and Vafa, Cumrun},
   year={2008},
   month={Feb},
   pages={106?106}
}
@article{Bastian_2018,
   title={Dual little strings and their partition functions},
   volume={97},
   ISSN={2470-0029},
   url={http://dx.doi.org/10.1103/PhysRevD.97.106004},
   DOI={10.1103/physrevd.97.106004},
   number={10},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Bastian, Brice and Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong},
   year={2018},
   month={May}
}
@article{Hohenegger_2020,
   title={From little string free energies towards modular graph functions},
   volume={2020},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP03(2020)077},
   DOI={10.1007/jhep03(2020)077},
   number={3},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Hohenegger, Stefan},
   year={2020},
   month={Mar}
}

@article{Bastian:2017ary,
    author = "Bastian, Brice and Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Triality in Little String Theories}",
    eprint = "1711.07921",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.97.046004",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "4",
    pages = "046004",
    year = "2018"
}
@article{Jefferson:2018irk,
    author = "Jefferson, Patrick and Katz, Sheldon and Kim, Hee-Cheol and Vafa, Cumrun",
    title = "{On Geometric Classification of 5d SCFTs}",
    eprint = "1801.04036",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP04(2018)103",
    journal = "JHEP",
    volume = "04",
    pages = "103",
    year = "2018"
}
@article{Hohenegger:2013ala,
    author = "Hohenegger, Stefan and Iqbal, Amer",
    title = "{M-strings, elliptic genera and $\mathcal{N} = 4$ string amplitudes}",
    eprint = "1310.1325",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-PH-TH-2013-237",
    doi = "10.1002/prop.201300035",
    journal = "Fortsch. Phys.",
    volume = "62",
    pages = "155--206",
    year = "2014"
}
@article{Hohenegger:2016yuv,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Dual Little Strings from F-Theory and Flop Transitions}",
    eprint = "1610.07916",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP07(2017)112",
    journal = "JHEP",
    volume = "07",
    pages = "112",
    year = "2017"
}

@article{Hohenegger:2015btj,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Instanton-monopole correspondence from M-branes on $\mathbb S^1$ and little string theory}",
    eprint = "1511.02787",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.93.066016",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "6",
    pages = "066016",
    year = "2016"
}

@article{Haghighat:2018gqf,
    author = "Haghighat, Babak and Sun, Rui",
    title = "{M5 branes and Theta Functions}",
    eprint = "1811.04938",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2019)192",
    journal = "JHEP",
    volume = "10",
    pages = "192",
    year = "2019"
}

@article{Bershadsky:1993cx,
    author = "Bershadsky, M. and Cecotti, S. and Ooguri, H. and Vafa, C.",
    title = "{Kodaira-Spencer theory of gravity and exact results for quantum string amplitudes}",
    eprint = "hep-th/9309140",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-93-A025, RIMS-946, SISSA-142-93-EP",
    doi = "10.1007/BF02099774",
    journal = "Commun. Math. Phys.",
    volume = "165",
    pages = "311--428",
    year = "1994"
}
@article{Ahmed:2017hfr,
    author = "Ahmed, Ambreen and Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{Bound states of little strings and symmetric orbifold conformal field theories}",
    eprint = "1706.04425",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.96.081901",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "8",
    pages = "081901",
    year = "2017"
}

@article{Hohenegger:2015cba,
    author = "Hohenegger, Stefan and Iqbal, Amer and Rey, Soo-Jong",
    title = "{M-strings, monopole strings, and modular forms}",
    eprint = "1503.06983",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SNUST-15-02",
    doi = "10.1103/PhysRevD.92.066005",
    journal = "Phys. Rev. D",
    volume = "92",
    number = "6",
    pages = "066005",
    year = "2015"
}

@article{Bousseau:2020ckw,
    author = "Bousseau, Pierrick and Fan, Honglu and Guo, Shuai and Wu, Longting",
    title = "{Holomorphic anomaly equation for $(\mathbb{P}^2,E)$ and the Nekrasov-Shatashvili limit of local $\mathbb{P}^2$}",
    eprint = "2001.05347",
    archivePrefix = "arXiv",
    primaryClass = "math.AG",
    month = "1",
    year = "2020"
}
@article{Liu:2005fz,
    author = "Liu, Chien-Hao and Yau, Shing-Tung",
    title = "{Transformation of algebraic Gromov-Witten invariants of three-folds under flops and small extremal transitions, with an appendix from the stringy and the symplectic viewpoint}",
    eprint = "math/0505084",
    archivePrefix = "arXiv",
    month = "4",
    year = "2005"
}

@article{Li:1998hba,
    author = "Li, An-Min and Ruan, Yongbin",
    title = "{Symplectic surgery and Gromov-Witten invariants of Calabi-Yau 3 folds. 1.}",
    eprint = "math/9803036",
    archivePrefix = "arXiv",
    month = "3",
    year = "1998"
}
@article{Gopakumar:1998jq,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 2.}",
    eprint = "hep-th/9812127",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A070",
    month = "12",
    year = "1998"
}

@article{Gopakumar:1998ii,
    author = "Gopakumar, Rajesh and Vafa, Cumrun",
    title = "{M theory and topological strings. 1.}",
    eprint = "hep-th/9809187",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-98-A069",
    month = "9",
    year = "1998"
}
@article{Kanazawa:2016tnt,
    author = "Kanazawa, Atsushi and Lau, Siu-Cheong",
    title = "{Local Calabi--Yau manifolds of type $\tilde A$ via SYZ mirror symmetry}",
    eprint = "1605.00342",
    archivePrefix = "arXiv",
    primaryClass = "math.AG",
    doi = "10.1016/j.geomphys.2018.12.015",
    journal = "J. Geom. Phys.",
    volume = "139",
    pages = "103--138",
    year = "2019"
}
   
@article{Harvey:2014nha,
    author = "Harvey, Jeffrey A. and Lee, Sungjay and Murthy, Sameer",
    title = "{Elliptic genera of ALE and ALF manifolds from gauged linear sigma models}",
    eprint = "1406.6342",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "EFI-14-10",
    doi = "10.1007/JHEP02(2015)110",
    journal = "JHEP",
    volume = "02",
    pages = "110",
    year = "2015"
}
@article{Marshakov:1999bw,
    author = "Marshakov, A.",
    title = "{Duality in integrable systems and generating functions for new Hamiltonians}",
    eprint = "hep-th/9912124",
    archivePrefix = "arXiv",
    reportNumber = "FIAN-TD-26-99, ITEP-TH-78-99",
    doi = "10.1016/S0370-2693(00)00076-9",
    journal = "Phys. Lett. B",
    volume = "476",
    pages = "420--426",
    year = "2000"
}

@article{Haghighat:2013gba,
    author = "Haghighat, Babak and Iqbal, Amer and Kozcaz, Can and Lockhart, Guglielmo and Vafa, Cumrun",
    title = "{M-Strings}",
    eprint = "1305.6322",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/s00220-014-2139-1",
    journal = "Commun. Math. Phys.",
    volume = "334",
    number = "2",
    pages = "779--842",
    year = "2015"
}
@article{Dijkgraaf:2007sw,
    author = "Dijkgraaf, Robbert and Hollands, Lotte and Sulkowski, Piotr and Vafa, Cumrun",
    title = "{Supersymmetric gauge theories, intersecting branes and free fermions}",
    eprint = "0709.4446",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "HUTP-07-A006, ITFA-2007-44, IFT-UW-2007-9",
    doi = "10.1088/1126-6708/2008/02/106",
    journal = "JHEP",
    volume = "02",
    pages = "106",
    year = "2008"
}
@article{DijkgraafR.1995,
  title={Mirror Symmetry and Elliptic Curves},
    author={Robbert Dijkgraaf },
%DOI :https://doi.org/10.1007
}

